A Diffusion-based Data Generator for Training Object Recognition Models in Ultra-Range Distance

Object recognition, commonly performed by a camera, is a fundamental requirement for robots to complete complex tasks. Some tasks require recognizing objects far from the robot's camera. A challenging example is Ultra-Range Gesture Recognition (URGR) in human-robot interaction where the user exhibits directive gestures at a distance of up to 25~m from the robot. However, training a model to recognize hardly visible objects located in ultra-range requires an exhaustive collection of a significant amount of labeled samples. The generation of synthetic training datasets is a recent solution to the lack of real-world data, while unable to properly replicate the realistic visual characteristics of distant objects in images. In this letter, we propose the Diffusion in Ultra-Range (DUR) framework based on a Diffusion model to generate labeled images of distant objects in various scenes. The DUR generator receives a desired distance and class (e.g., gesture) and outputs a corresponding synthetic image. We apply DUR to train a URGR model with directive gestures in which fine details of the gesturing hand are challenging to distinguish. DUR is compared to other types of generative models showcasing superiority both in fidelity and in recognition success rate when training a URGR model. More importantly, training a DUR model on a limited amount of real data and then using it to generate synthetic data for training a URGR model outperforms directly training the URGR model on real data. The synthetic-based URGR model is also demonstrated in gesture-based direction of a ground robot.

==> GAN.tex <==
Generative Adversarial Networks (GANs) \cite{goodfellow2014generative} have revolutionized the landscape of artificial intelligence, introducing an intricate interplay between generative models and their discriminative counterparts. This foundational concept has paved the way for the evolution of Conditional GANs (cGANs) \cite{mirza2014conditional}, an augmentation that strategically incorporates conditional variables, such as class labels, affording meticulous control over the generative process and thereby facilitating the targeted synthesis of data endowed with predefined attributes. In tandem, the pioneering Progressive Growth of GANs methodology, as advanced \cite{karras2017progressive}. It has had a profound impact on the training dynamics of GANs. By systematically and progressively elevating image resolution throughout the course of training, this innovative approach has yielded a confluence of benefits, encompassing heightened training stability, amplified image fidelity, and enriched diversity. This transformative progression stands as a testament to the iterative refinement of GAN techniques, contributing substantively to improved quality, enhanced stability, and augmented variation in the synthesized outputs. 

This paper presents an initiative to construct an innovative database through the integration of a conditional progressive GAN framework. Our objective centers on the establishment of both a Distance GAN and Gesture GAN. These models are designed to proficiently generate user, strategically varying in distance while adhering to designated distance conditions, alongside distinct gestures. This endeavor assumes paramount significance in furnishing synthetic data for the purpose of model training. The confluence of these attributes serves as a pivotal resource, empowering our model with the discernment of diverse proximities and intricate gestural manifestations. Our motivation underscores the imperative of addressing the paucity of datasets that holistically encompass these dual attributes, thereby augmenting the veracity and depth of training data.

\subsection{Gestures and distance Gan}
\label{sec:Synthetic}

Over the past years, the field of Generative Adversarial Networks (GANs) has witnessed significant developments, leading to the emergence of numerous GAN-based applications and techniques for synthetic data generation. These advancements, which either incorporate GAN technology or are directly influenced by GAN principles, have broadened the horizons of synthetic data creation.
Primarily, GANs have been utilized to produce synthetic images and matrices. However, it is important to note that images generated through GANs typically exhibit low resolutions and tend to emphasize a single central object within the synthetic image. To the best of our knowledge, there exists a conspicuous dearth of research addressing the generation of complex images containing multiple objects within the frame, where no single object is the exclusive focal point.

Our research aims to address this void by developing a GAN model capable of generating diverse synthetic data characterized by complex frames containing multiple objects. Furthermore, we seek to diversify our synthetic data by incorporating various environmental settings, different individuals, and distinct weather conditions, encompassing a variety of lighting scenarios. Additionally, our model will account for different gestures made by the individuals and variations in their distance from the camera.
The development of such a GAN model holds significant promise, as it can serve as a simulator capable of producing synthetic data that closely approximates the characteristics of real-world data acquired across diverse environments. This endeavor offers several advantages, including reducing the need for extensive data collection ($\text{Data Reduction}$), mitigating equipment constraints ($\text{Equipment Constraints}$), facilitating the training of new models ($\text{Model Training}$), and enabling the exploration of novel tasks ($\text{Novel Tasks}$). This becomes especially advantageous when additional data production is required ($\text{Increased Data Demand}$), and human resources are limited ($\text{Resource Constraints}$).

In this research, we strive to create a GAN model that incorporates distance and gesture conditions, with the objective of demonstrating its efficacy in generating complex images under varying conditions and gestures ($\text{GAN Performance}$). Through this effort, we aim to make a substantial contribution to the field of synthetic data generation ($\text{Research Contribution}$) and its applicability across a wide spectrum of challenging image scenarios ($\text{Image Generation}$).

We employed a neural network architecture that combines the U-Net structure with the capacity for conditional image generation. This variant of the U-Net architecture is specifically engineered to produce images contingent upon particular conditions, such as human gestures (\( G \)) and the distance of the human subject from the camera (\( D \)).

Conditional image generation is a paradigm where the network incorporates additional information, denoted as conditions (\( C \)), during the image generation process. These conditions serve as guiding factors, enabling the network to generate images that conform to specific criteria. In our context, we endeavored to set our conditions as follows: \( C = \{2 \leq D \leq 20\, \text{meters}, G \in \text{six human gestures}\} \).

To achieve this, we harnessed the power of the Disentangled Conditional Diffusion Model based on Gaussian noise (DCDM-G) \cite{mao2023disc}. In general, Diffusion models are based on the concept of simulating the diffusion process, where noise is added to an image and recover the original image from the noisy version. This specific architectural innovation amalgamates disentangled conditional generation with a Gaussian diffusion process for image generation. The DCDM-G model is defined by:

\[
p(x | C) = \int p(x | z, C) p(z | C) dz
\]

Here, \( x \) represents the generated image, \( C \) signifies the conditional information (in our case, \( C = \{D, G\} \)), and \( z \) is the latent variable.

The strength of DCDM-G lies in its ability to produce images that disentangle and control specific attributes (\( D \) and \( G \)) based on conditional input, all while ensuring that the generated images adhere to the desired data distribution. This makes it a formidable tool for generating images with finely controlled features, such as human gestures at varying distances from the camera.


==> relatedwork.tex <==



Several studies have investigated the use of synthetic data techniques for recognizing human gestures. One popular approach is to develop an algorithm to render a palm in a 3D simulator such that it appears in several positions or makes several sequential movements. Another approach is the use of GAN in order to generate images of a gesturing palm, or simulate a skeleton movements. 

In \cite{de2020vision} research they use a commercial game engine, namely Unity, to create synthetic videos of human gestures, in addition to real videos with human subjects. The synthetic and real videos both display a full human body, however, no distance from the "camera" was specified. In order to classify the recorded gesture, they use their model that is based on the Inflated 3D convolutional (I3D) network that was developed formerly. 

Other researches propose to focus on a human palm only. \cite{Tsai8252982} use of the open source 3D graphics package Blender to create the 3D skeleton of a hand, following the dynamic joints constraints of each finger. By doing so, synthetic images of hands can be used to represent real images captured by a live camera. Alongside true RGB images of a human hand, they trained a deep CNN model for recognition of the represented gesture. 

In \cite{tu2021fingerspelling} they also use Blender software to render a hand in order to recognize  fingerspelling signs. In addition to that, they propose the use of Neural Style Transfer (NST) in order to add texture to the rendered hand, and thus increases the diversity of the data. Although \cite{cai2018weakly} focuses on hand pose estimation rather than recognizing the gesture, the use of Rendered Hand Pose Dataset (RHD), as an additional dataset to the real-world one, is also effective in regression tasks. 

In \cite{molina2014natural}, for generating synthetic data, they use a hand skeleton model and added a volumetric hand via a morphological dilation process. Unlike previously mentioned researches, this synthetic data was added to real hand images that were taken by Time-Of-Flight (TOF) cameras, and not by regular RGB cameras, adding a third dimension to the image as a consequence. In terms of recognition, they used pose-based separability method to separate a set of gestures, with no need of applying classification techniques. 


\cite{sabbarese2023hand} \hl{bad citation} use public datasets of human gestures, taken by a regular RGB cameres and at short distances. Additionally, a synthetic dataset was generated by utilizing RealSense sensors, which was then replicated by a behavioral tree simulation application, which mapped these gestures onto 3D hand models and generated frames with varying backgrounds, positions, distances, and rotations. For gesture recognition, they use Hand Tracking module and MediaPipe's hand landmarks applied to each frame, then an RNN modle is used, comprised two layers of either LSTM or GRU and a Fully Connected output layer.

The utilization of Generative Adversarial Network (GAN) for creating synthetic data for gesture recognition was proposed by \cite{fang2019gesture} and \cite{zhou2022lightweight}. In order to isolate the hand from the background, they used a semantic segmentation technique, thus turning images into binary images. Due to the diversity created by the synthetic data, the overfitting problem for the recognition model was solved.

In \cite{liu2019improved} they also isolated the palm from the background by segmentation, however, their dataset includes synchronized depth and color of the hand region in order to accurately capture the hand movements in both modalities. With this in mind, they used an Image-to-Image Translation with Conditional Adversarial networks (pix2pix) to generate pseudo-depth hand data  to improve the in RGB-only hand gestures recognition performance. In the recognition phase, they propose a two-stream CNN architecture with color image and its pseudo depth image.



Another approach for gesture recognition problem is, instead of using images of a hand or a person, Shen et al. \cite{shen2021imaginative} use solely skeleton-based datasets. By using Imaginative GAN, they sample new data from the distribution of the input data, and thus augmenting the whole dataset and improving the classification accuracy as a consequence. In their study, they compared the use of Imaginative GAN with classical data augmentation methods, which include changes in scale, displacement, time interpolation, and noise to every data point. They found that Imaginative GAN performed better than classical augmentation methods, measured by mean validation accuracy, standard error, and time cost to find an optimized strategy.

To the best of our knowledge, the distance between participants and the camera did not exceed 3 meters, as delineated in Table \ref{tb:sota}, since gesture recognition predominantly centered around the palm shape or its movements. Furthermore, most of the methods mentioned above tried to isolate the hand from the background, which is more difficult when dealing with longer distances, since the pixels of the hand sometimes blend with the pixels of the environment.


\begin{table*}
    \centering
    \caption{State-of-the-art comparison of recognition methods using synthetic data}
    \label{tb:sota}
    \begin{tabular}{l|cccccccc}
        & Recognition & Skeleton & Segmentation & Distance [m] & Indoor & Outdoor & RGB/Depth & \textbf{G}AN/ \textbf{D}iffusion/  \\     
        
        Paper & & &&& & & & \textbf{S}imulator \\\hline
        
        de Melo et al. \cite{de2020vision} & \checkmark & \xmark & \xmark &  - & \xmark & \checkmark & RGB & S \\

        Zhou et al. \cite{zhou2022lightweight} & \checkmark & \xmark & \checkmark &  - & \checkmark & \xmark & RGB &  G \\

        Molina et al. \cite{molina2014natural} & \checkmark & \xmark & \xmark &  3 & \checkmark & \xmark & Depth & S \\

        Tsai et al. \cite{Tsai8252982} & \checkmark & \xmark & \xmark &  - & \checkmark & \xmark & RGB & S \\

        Fang et al. \cite{fang2019gesture} & \checkmark & \xmark & \checkmark &  - & \checkmark & \xmark & RGB & G \\

        Liu et al. \cite{liu2019improved} & \checkmark & \xmark & \checkmark & - & \checkmark & \xmark & RGB & G \\

        Tu et al. \cite{tu2021fingerspelling} & \checkmark & \xmark & \xmark &  - & \checkmark & \xmark & RGB & S \\

        Shen et al. \cite{shen2021imaginative }& \checkmark & \checkmark & \xmark &  - & - & - & - & G \\

        Cai et al. \cite{cai2018weakly} & \xmark & \checkmark & \xmark &  - & \checkmark & \xmark & RGB & S \\

        Sabbarese et al. \cite{sabbarese2023hand} & \checkmark & \checkmark & \xmark &  - & \checkmark & \xmark & RGB & S \\
        
        
        \hline
        Proposed method & \checkmark & \xmark & \xmark & 20 & \checkmark & \checkmark & RGB & D \\    \hline
    \end{tabular}
    % \begin{tablenotes}

    % \end{tablenotes}
\end{table*}

























